Towards Top-Down Automated Development in Limited Scopes: A Neuro-Symbolic Framework from Expressibles to Executables

Deep code generation is a topic of deep learning for software engineering (DL4SE), which adopts neural models to generate code for the intended functions. Since end-to-end neural methods lack domain knowledge and software hierarchy awareness, they tend to perform poorly w.r.t project-level tasks. To systematically explore the potential improvements of code generation, we let it participate in the whole top-down development from \emph{expressibles} to \emph{executables}, which is possible in limited scopes. In the process, it benefits from massive samples, features, and knowledge. As the foundation, we suggest building a taxonomy on code data, namely code taxonomy, leveraging the categorization of code information. Moreover, we introduce a three-layer semantic pyramid (SP) to associate text data and code data. It identifies the information of different abstraction levels, and thus introduces the domain knowledge on development and reveals the hierarchy of software. Furthermore, we propose a semantic pyramid framework (SPF) as the approach, focusing on software of high modularity and low complexity. SPF divides the code generation process into stages and reserves spots for potential interactions. In addition, we conceived preliminary applications in software development to confirm the neuro-symbolic framework.

==> listings/demo.tex <==
\begin{lstlisting}[language=Java,label={lst:demo},caption=A Code Snippet in Java]
/**
* Check birthday and return Happy Birthday message
*/
public String getBirthdayGreetings() {
    // declare variables for birthday
    int birthDate = 3;
    Month birthMonth = Month.JANUARY;
    // get current date and month
    LocalDate currentDate = LocalDate.now();
    int date = currentDate.getDayOfMonth();
    Month month = currentDate.getMonth();

    if(date == birthDate && month == birthMonth)
        return "HAPPY BIRTHDAY TO YOU";
    return None;
}
\end{lstlisting}
